Optimizing Tree-structure Indexes for CXL-based Heterogeneous Memory with SINLK

On heterogeneous memory (HM) where fast memory (i.e., CPU-attached DRAM) and slow memory (e.g., remote NUMA memory, RDMA-connected memory, Persistent Memory (PM)) coexist, optimizing the placement of tree-structure indexes (e.g., B+tree) is crucial to achieving high performance while enjoying memory expansion. Nowadays, CXL-based heterogeneous memory (CXL-HM) is emerging due to its high efficiency and memory semantics. Prior tree-structure index placement schemes for HM cannot effectively boost performance on CXL-HM, as they fail to adapt to the changes in hardware characteristics and semantics. Additionally, existing CXL-HM page-level data placement schemes are not efficient for tree-structure indexes due to the granularity mismatch between the tree nodes and the page. In this paper, we argue for a CXL native, tree-structure aware data placement scheme to optimize tree-structure indexes on CXL-HM. Our key insight is that the placement of tree-structure indexes on CXL-HM should match the tree's inherent characteristics with CXL-HM features. We present SINLK, a tree-structure aware, node-grained data placement scheme for tree-structure indexes on CXL-HM. With SINLK, developers can easily adapt existing tree-structure indexes to CXL-HM. We have integrated the B+tree and radix tree with SINLK to demonstrate its effectiveness. Evaluations show that SINLK improves throughput by up to 71% and reduces P99 latency by up to 81% compared with state-of-the-art data placement schemes (e.g., MEMTIS) and HM-optimized tree-structure indexes in YCSB and real-world workloads.

==> design.tex <==
\section{Overview of {\sys}}%
\label{sec:design}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{./figures/arch.pdf}
    \vspace{-10pt}
    \caption{\textbf{Architecture and interactions of {\sys}.}{ PQ stands for promotion queue, DQ stands for demotion queue.}}%
    \label{fig:high-level-arch}
    \vspace{-15pt}
\end{figure}

To solve the challenges in \autoref{sec:challenge}, we design {\sys}, an efficient and generic data placement scheme for tree-structure indexes on {\chm}.
As depicted in \autoref{fig:high-level-arch}, {\sys} consists of a lightweight frontend module and a background module.


\noindent
\textbf{The frontend module} is invoked in the critical path of the tree's operations so that it is designed to be lightweight to minimize the impact on the tree's performance.
It determines the initial position of a new node (\ding{182}) to ensure the \emph{single-boundary structure}.
The frontend module is also responsible for updating leaf nodes' access frequency (\ding{183}), laying the groundwork for hot path identification.


\noindent
\textbf{The background module} consists of several background workers to conduct node migration (\autoref{sub:migration}) and system adjustment (\autoref{sub:watermark}) to optimize fast memory usage asynchronously.
The \emph{migration trigger} decides whether migration is needed and picks the appropriate nodes for migration based on their access frequency (\ding{184}) and the distribution (i.e., the histogram) of all nodes' access frequency (\ding{185}).
The \emph{promotion executor} and \emph{demotion executor} get nodes from the corresponding queues and carry out the migration tasks (\ding{186}).
The \emph{cooler} periodically halves the nodes' access frequency (\ding{187}) to ensure the freshness of access information.
To coordinate all workers, the \emph{watermark maintainer} tracks the fast memory usage and adjusts system parameters and workers' execution to efficiently ensure optimal utilization of fast memory (\ding{188}).


























==> framework.tex <==
\section{{\sys} Framework}%
\label{sec:framework}

\makeatletter
\lst@InstallKeywords k{attributes}{attributestyle}\slshape{attributestyle}{}ld
\makeatother


We provide a lightweight and easy-to-use framework for integrating {\sys} into various existing tree-structure indexes\footnote{Details of the framework and user guide are provided in \autoref{sec:appendix}.}.
Regarding {\sys} metadata, the framework requires developers to add one byte to the internal node to record the node's level and memory type, and for leaf nodes, two additional bytes are needed to store the access frequency.
For the frontend module, {\sys} framework provides several helper functions that implement layer-aware allocation and leaf-centric access tracking for developers to use.
Additionally, developers need to implement tree-specific logic in the interfaces defined within {\sys} framework to enable the background module to interact with the tree.
Notably, while {\sys} requires some user-implemented functions, many of them can draw on or utilize the existing tree logic, such as node splitting for migration and iterators for traversing leaves.
 

